Improving generalisability of 3D binding affinity models in low data regimes

Predicting protein-ligand binding affinity is an essential part of computer-aided drug design. However, generalisable and performant global binding affinity models remain elusive, particularly in low data regimes. Despite the evolution of model architectures, current benchmarks are not well-suited to probe the generalisability of 3D binding affinity models. Furthermore, 3D global architectures such as GNNs have not lived up to performance expectations. To investigate these issues, we introduce a novel split of the PDBBind dataset, minimizing similarity leakage between train and test sets and allowing for a fair and direct comparison between various model architectures. On this low similarity split, we demonstrate that, in general, 3D global models are superior to protein-specific local models in low data regimes. We also demonstrate that the performance of GNNs benefits from three novel contributions: supervised pre-training via quantum mechanical data, unsupervised pre-training via small molecule diffusion, and explicitly modeling hydrogen atoms in the input graph. We believe that this work introduces promising new approaches to unlock the potential of GNN architectures for binding affinity modelling.

==> sections/1_introduction_short.tex <==
\section{Introduction}
% Say why binding affinity prediction is important and where this is used.
Computer-aided drug design relies on the accurate prediction of protein-ligand binding affinity to achieve a therapeutic effect, ensuring selectivity against other proteins and avoiding off-target toxicity \citep{kairys2019binding}.

The majority of the literature indicates that it is still unclear whether a specific model type consistently achieves the best results \citep{durant2023robustly}. Part of this ambiguity is due to the lack of consistent benchmarks to evaluate the performance of the diverse array of models. The common dataset used for benchmarking 3D binding affinity models is the \pdbbind \citep{liu2015pdbbind}, a dataset of crystal structures from the Protein Data Bank (PDB) with curated binding affinity measurements. Over the last few years, many splits have been proposed for the \pdbbind dataset to probe performance and generalisation of different model types \citep{volkov2022frustration,durant2023robustly,li2024leakproofpdbbindreorganized}, but each come with their own drawbacks. 
On the whole, the results suggest that simpler models and baselines perform just as well as the more complicated 3D models that use structural information \citep{durant2023robustly}. This implies that 3D models are not learning generalizable information but only dataset biases, hence they have not yet met their projected expectations \citep{volkov2022frustration}.

In this work we investigate the performance of binding affinity model families in a robust setting to probe what they learn and how they generalise. We compare 3D global models to protein-specific local models commonly used in real world drug discovery and also to baseline bias models. To achieve this, we propose a new split of the \pdbbind dataset based on protein and ligand similarity and constructed to suit bechmarking the various model families fairly and consistently. 
We use the new split and strong baselines to test multiple novel improvements to a plain 3D GNN model to push the boundaries of binding affinity modelling using 3D GNNs. 


==> sections/2_methods_short.tex <==
\section{Methods}

In this section, we present an overview of our methods and benchmarks. We have made the code, prepared structures, and splits in this work publicly available at \lowsimgithub and \ccdczenodo.

\subsection{\pdbbind dataset}
We choose the \pdbbind dataset (release v2020\footnote{As of 2024, there is a newer \pdbbind release (v2021) available at \url{https://www.pdbbind-plus.org.cn/}. We did not use it in this work, as access is restricted.}) as our benchmarking data set \citep{liu2015pdbbind}. To prepare the dataset, we queried the PDB \citep{wwpdb2019protein} for biological assemblies of all the structures listed in the \pdbbind dataset. To address both of these issues, each structure was prepared using CCDC software \citep{groom2016cambridge}, namely the Python API (\texttt{v.3.0.16}). Hydrogen atoms were added and the ligands listed by \pdbbind as biologically relevant were extracted into separate files. The remaining ligands of non-biological nature along with water molecules were removed. After preparation, 18,310 structures out of the total 19,443 remained (1,133 failed).


\subsection{Models}

Next, we discuss the models used in this study. An overview is presented in \tabref{table::models}. A full description of the hyperparameters of the features and models is provided in the Supplementary Information.

\begin{table}[h]  
\centering  
\caption{Overview of the different models used in this study. We indicate whether the models are global or local and whether they use 3D information or not. We make use of two baseline models to estimate dataset biases (\ligandbias and \mw).}  
\begin{tabular}{lccc}  
\toprule  
\textbf{Model Name} & \textbf{Global/Local} & \textbf{3D/non-3D} & \textbf{Input} \\  
\midrule  
\singleprotein & local & non-3D & ligand only \\ 

EGNN \citep{satorras2022enequivariantgraphneuralegnn}& global & 3D & pocket + ligand \\  
\rfscore \citep{ballester2010rfscore} & global & 3D & pocket + ligand \\  
\onion \citep{Wang2021onionnet2} & global & 3D & pocket + ligand    \\
\cmidrule(lr){1-4}
\ligandbias & global & non-3D & ligand only \\
\mw & local & non-3D & ligand  only \\
\bottomrule  
\end{tabular}
\label{table::models}
\end{table}

\paragraph{Model families}
We categorise the models by the scope of application, global vs. local, and the type of data input, non-3D vs. 3D. We denote models intended for use on different protein targets by \textbf{global models} and ones intended for use against a single protein target by \textbf{local models}. We further denote models which do not use 3D coordinates by \textbf{non-3D models} and ones which do by \textbf{3D models}.


\paragraph{\singleprotein local models}
\label{sec:methods:single_protein_local_models}
To compare to standard practices in the drug discovery community and in real world projects \citep{lo2018machine}, we benchmark the performance of \singleprotein local models built from ligand-based features and trained on binding activity data measured against a single protein. Analogous to established workflows \citep{jiang2021could,deng2023systematic}, we use classical machine learning models (Random Forest \citep{breiman2001randomforests}, XGBoost \citep{chen2016xgboost}, CatBoost \citep{prokhorenkova2018catboost}, Support Vector Machine \citep{cortes1995support}) combined with a selection of fingerprints (ECFP, FCFP, atom pairs, topological torsion) and molecular descriptors for features.


\paragraph{EGNN models}
We use the EGNN \citep{satorras2022enequivariantgraphneuralegnn} model as the base architecture for our 3D global models. We use the implementation in the \physicsml python package \anonref{physicsml}. As in previous work, we extract the protein pocket by selecting protein atoms within 5\AA\ of any ligand atom. The graph is constructed from the pocket and ligand atoms as nodes and a 5\AA\ cut-off is used to define the edges. We use one-hot encoded atomic numbers as node features and no edge features.

In addition to the basic model, we use two pre-trained versions.\footnote{Information about both pre-training strategies and transfer learning is available in the Supplementary Information.} The \textbf{EGNN-QM} model is trained on ANI1ccx, a dataset of approximately 500k small molecules with quantum mechanical energies computed at the ccsd(t) level. The \textbf{EGNN-DIFF} model is trained as a small molecule diffusion model on the QM9 dataset (as described in \cite{pmlr-v162-hoogeboom22a}). Since hydrogen atoms contribute significantly to binding via hydrogen bonds, we benchmark the models with no hydrogen atoms (\textbf{None}), with only the polar hydrogen atoms (\textbf{Polar}), and with all hydrogens (\textbf{Explicit}). Finally, to probe whether the models learn to identify the interactions from the protein-ligand pose, we also train models on the pockets and ligands as separate graphs. We refer to models which treat proteins and ligands as separate graphs by \textbf{\multigraph} models and the models that operate on the interacting pose by \textbf{\singlegraph} models.

% Models which use the interacting pose are termed \textbf{\singlegraph} models, with those using the protein and ligand as separate graphs denoted as \textbf{\multigraph} models.
\paragraph{\rfscore and \onion}
We include in our analysis two additional 3D global models, \rfscore and \onion. We select those models due to their performance on other splits of the \pdbbind dataset as indicated in the study by \cite{durant2023robustly}. Specifically, \rfscore was one of the top performers on the CASF-2016 split, while the \onion model was superior on the 2019-Holdout and Peptides-Holdout sets relative to other models tested.

\paragraph{Baseline models}
To probe the ligand dataset bias in the benchmarking splits, we follow the work of \cite{durant2023robustly} and design a \ligandbias global model. This model is trained on the identical data used to train the global models (binding affinity measurements of ligands against different proteins), but only uses ligand-based features as input (analogous to \singleprotein models; see \ref{sec:methods:single_protein_local_models}). Effectively, this mixes binding affinity values of compounds measured against different proteins to probe the amount of dataset bias available in ligand information alone. We also employ a \mw model that uses the molecular weight of the ligand as its sole input as a baseline. We use the same architectures and training data as for the \singleprotein local models.

\subsection{Splitting}
We propose a new split of \pdbbind based on protein and ligand similarity, which we call the \textbf{\oursplit} split. Although many splits have been proposed, we believe that none achieve our goal of probing generalisation. Close inspection of the proposed splits \citep{volkov2022frustration,durant2023robustly,li2024leakproofpdbbindreorganized} shows non-negligible levels of similarity between train and test set, with all splits sharing some proteins (UniProts) across sets. Furthermore, the splits were not constructed to benchmark the variety of model families available (local vs. global, 3D vs. non-3D).

We design our splits such that we can compare between global and local models. This comparison is particularly relevant given that local \singleprotein models are still widely used in drug discovery projects. We select eight proteins from the \pdbbind dataset which have more than 100 datapoints as our case study. The threshold of 100 points per protein is to allow enough data to train local models. In total, the \casestudy consists of 1,857 structures. These proteins will be used to benchmark the generalisability of global models and also to train local models for each specific protein. We compute the similarity to the \casestudy using FoldSeek \citep{Van_Kempen2024-ql-foldseek}. We filter out any structures which have more than 0.5 similarity to the \casestudy structures. Additionally, we compute the tanimoto similarity between the \casestudy ligands and the ligands of the remaining structures. We filter out any structures with ligands with more than 0.5 tanimoto similarity. A total of 5,431 similar structures are removed and leaves 11,022 structures in the \otherproteins set.

We use the \oursplit split (1,875 \casestudy structures and 11,022 \otherproteins structures) to construct the benchmarking splits as follows. We stratify the \casestudy data by protein and split the structures by tanimoto ligand similarity with increasing fraction of training data, 5\%, 30\%, 80\%. At each percentage, we generate three folds with a different starting seed ligand for the similarity splits. Local models are trained on these splits for each protein individually. For the global models, we further augment the train sets of these splits with the \otherproteins. Additionally, we construct the 0\% split where all \casestudy are in the test set and only the \otherproteins are in the train set. This is to probe generalisation to completely new proteins. The final benchmarking splits are shown schematically in Figure~\ref{fig::splits_and_results} on the left. In absolute numbers, those splits correspond to the following number of training samples per protein: 11$\pm$5 (5\%), 69$\pm$30 (30\%), 185$\pm$83 (80\%).


\begin{figure}
  \begin{minipage}[t]{.49\linewidth}
    \vspace{0pt}
    \includegraphics[width=\textwidth]{plots/split_figure.png} 
  \end{minipage}
  \begin{minipage}[t]{.49\linewidth}
    \vspace{1pt}
    \includegraphics[width=\textwidth]{plots/overall_r2.png} 
  \end{minipage}
      \caption{Left: Schematic of \oursplit split. Global models are trained on both train sets from the \casestudy and the \otherproteins. Local models are individually built for each of the eight proteins in the \casestudy split. Right: Overall performance of models. In the low data regime, global 3D models outperform local models. The error bars denote the standard deviation across the three test folds. In the 0\% split case, there is a only a single test fold. Due to the non-deterministic nature of training, variation in performance is due to training the same ML models three times. No local models can be built for the 0\% split.}
\label{fig::splits_and_results}
\end{figure}

\subsection{Metrics}
Typically, binding affinity models are assessed using the Pearson correlation coefficient, which measures the correlation between predicted and actual binding affinity values. However, this doesn't measure the absolute predictive performance, which is crucial in real-world drug discovery for optimising multi-parameter objectives. Therefore, here we focus on the absolute $R^2$ metric for benchmarking performance, while also providing root mean squared error and Pearson correlation results in the Supplementary Information.

==> sections/3_results_short.tex <==
\section{Results}

% We now present the results of the benchmarking. First, we present the results and comparisons across model families. We follow this with more detailed analyses of the 3D EGNN models.

\subsection{Model family comparisons}

The results reveal a clear advantage for global 3D models over local models in low data regimes. As seen in Figure \ref{fig::splits_and_results} on the right, the global 3D models have moderate generalisation even with 0\% protein-specific training data and outperform the \singleprotein model at lower train data fractions (5\% and 30\%). With enough data (80\%), most models plateau at similar performance. We hypothesise that this is due to the difficulty of the tanimoto similarity splits. At low data levels, the local models not only have very little data to learn from but also a train set which is very dissimilar to the test ligands. In drug discovery settings where generalisation is important, this benchmark clearly highlights the importance of global models. Notably, the pre-trained EGNN models outperform all other models and baselines when considering the overall performance (Figure \ref{fig::splits_and_results}, left). See \secref{subsec::EGNN_additions} for a detailed analysis of their performance.

One thing to note is the relatively good performance of the \ligandbias model (red bar in Figure~\ref{fig::splits_and_results}, right). Although not as good as the global 3D models, the \ligandbias model is able to generalise to the unseen proteins. We hypothesise that this is due to the model picking up on functional group importance in the ligands, given that a lot of binders rely on generic functional groups.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\textwidth]{plots/gnn_combined_r2.png} 
  \caption{Effect of the EGNN additions proposed in this study on model performance. The overall performance across all eight proteins in the \casestudy set is reported. The error bars denote the standard deviation across the three test folds. In the 0\% split case, there is a only a single test fold. Due to the non-deterministic nature of training, variation in performance is due to training the same EGNN model three times. \textbf{Pre-training}: Quantum mechanical pre-training provides the greatest advantage, followed closely by diffusion pre-training.
  \textbf{Hydrogens}: Including explicit hydrogens is very important at low data levels.
  \textbf{Interacting pose}: No consistent pattern when comparing single-graph versus multi-graph. }
  \label{fig::gnn-benchmarks}
\end{figure}

\subsection{Improvements to EGNNs}
\label{subsec::EGNN_additions}

As Figure~\ref{fig::gnn-benchmarks} (left) shows, pre-training significantly improves model performance. Quantum mechanical pre-training provides the largest advantage followed closely by diffusion pre-training. As expected, the advantages are more noticeable at low levels of training data, gradually fading out as more training data is added. To our knowledge, this is the first application of using pre-trained models for 3D binding affinity prediction.

Next, we assess the effect of including hydrogen atoms on model performance. To our knowledge, in all previously published work, hydrogen atoms were ignored in the structures. As can be seen in Figure \ref{fig::gnn-benchmarks} (middle), hydrogens are very import at low data levels for generalisation. With more data, their effect becomes negligible. This is very important to keep in-mind for building models that generalise to new proteins and novel ligand chemical space. The newly proposed encoding introduced in this study can be directly applied, given that the CCDC in 2023 released a curated dataset of protein structures from the PDB with hydrogen atoms added \citep{ccdcstructures}.

Finally, we look at the effect of the interacting pose on performance. As we can see in Figure \ref{fig::gnn-benchmarks} on the right, using the pose information (single-graph model) does not necessarily improve the model performance. Further investigation is required to understand what the models are learning. 


==> sections/4_discussion_short.tex <==
\section{Discussion}

In this paper, we demonstrate that for binding affinity prediction on new proteins and chemical spaces, global 3D models outperform local models on the \pdbbind dataset. Furthermore, we show that explicit hydrogen atoms in the structures and novel pre-training strategies using quantum mechanical data and diffusion modelling provide performance improvements in low data regimes for GNNs.

There are limitations to the above benchmark. This work focuses on the \pdbbind dataset, a dataset comprising only crystal structures. We explicitly chose to do so to eliminate any sources of noise or error from computationally generated structures and poses. However, this has two drawbacks. First, the structures and chemical space of ligands in the dataset are not representative of the distribution of ligands in a real-world drug discovery projects. The relatively good performance of the \ligandbias model indicates the lack of diversity in the ligand distribution. Second, since crystal structures can only be obtained for binding ligands, this benchmark does not probe the performance of models for non-binding ligands. This is important for virtual high throughput screens where many ligands might not be binders.

In light of these limitations, it is crucial to replicate a similar analysis on additional datasets, ideally resembling real-world drug discovery datasets. If insights from this study are confirmed with more datasets, this research could represent a significant stride towards developing more universally applicable 3D binding affinity models that leverage pre-training strategies.




% Finally, even though we filter the dataset for UniProt and similarity overlap, we noticed that there are still shared protein families in the train and test sets. We aim to improve this in future work.

==> sections/6_neurips_paper_checklist.tex <==
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide experiments, results, and discussion of the claims in the abstract and introduction. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: In the Discussion, we provide and overview of the limitations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: No theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: We discuss the approach in detail and make the code and data available.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide access to the data and code and provide instructions on how to use them and reproduce the results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide detailed explanation of the splits and make them available with the code and data release.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: We validate our results with multiple repeats and provide error bars to denote the statistical significance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide this information in the Supplementary Information
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerNA{}
    \item[] Justification: No particular ethics concerns
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}, \answerNo{}
    \item[] Justification: All creators are credited when required.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide instructions on how to use the code and data in the code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/supplementary_info_short.tex <==
\begin{center}
\textbf{\large Supplemental Information}
\end{center}

\section{\singleprotein hyperparameters}

We used classical architectures and features for the \singleprotein models. All the models and features below can be found in the python package \molflux (\anonref{molflux}).

\begin{table}[h]  
\centering  
\caption{\singleprotein models}  
\begin{tabular}{lccc}  
\toprule  
\textbf{Model Name} & \textbf{hyperparameters}\\  
\midrule  
Random Forest & $\mathtt{n\_ estimators}=500$ \\
\midrule  
XGBoost & \makecell{$\mathtt{learning\_ rate}=0.2$ \\ $\mathtt{subsample}=1$ \\ $\mathtt{max\_ depth}=6$} \\
\midrule  
CatBoost & $\mathtt{random\_ state}=0$ \\
\midrule  
Support Vector Regressor & $\mathtt{kernel}=\mathtt{rbf}$ \\
\bottomrule  
\end{tabular}  
\end{table}

\begin{table}[h]  
\centering  
\caption{\singleprotein features}  
\begin{tabular}{lccc}  
\toprule  
\textbf{Feature name} & \textbf{Comments}\\  
\midrule  
Molecular Weight &  \\
\midrule  
Molecular descriptors (MD) & \makecell{xLogP, aromatic ring count \\ molecular weight, num acceptors \\ num donors, rotatable bonds, tpsa \\  \\ All descriptors were normalised  \\ by the train set mean and variance}\\
\midrule  
ECFP & circular 2048 fingerprints \\
\midrule  
FCFP & \\
\midrule  
Topological torsion & \\
\midrule  
ECFP + MD &  \\
\midrule  
FCFP + MD &  \\
\midrule  
Topological torsion + MD & \\
\bottomrule  
\end{tabular}  
\end{table}

\section{EGNN models}

We used the following hyperparameters for the EGNN models.

\begin{table}[h]  
\centering  
\caption{\singleprotein models}  
\begin{tabular}{lccc}  
\toprule  
\textbf{Hyperparameter} & Value \\  
\midrule  
$\text{num}\_\text{layers}$ & 5 \\
$\text{c}\_\text{hidden}$ & 128 \\
$\text{num}\_\text{rbf}$ & 8 \\
$\text{pool}\_\text{type}$ & sum \\
Activation & SiLU \\
Loss & MSELoss \\
Optimizer & AdamW, LR$=5\times10^{-4}$ \\
Scheduler & ReduceLROnPlateau \\
\bottomrule  
\end{tabular}  
\end{table}

\section{Pre-training EGNN models}

\subsection{Quantum mechanical energy}

The EGNN-QM model was pre-trained on the ccsd(t) energy of the ANI1ccx dataset. This is a dataset of roughly 500k small molecules. As is common in the domain of neural network potentials, the model was trained to predict the interaction energy (the total energy minus the self atomic energies of the atoms). The final root mean squared error of the model was 4kcal/mol. 

\subsection{Small molecule diffusion}

The EGNN-DIFF model was trained to generate small molecules from the QM9 dataset (small molecule with up to 9 heavy atoms). This was carried out as described in the original work by \cite{pmlr-v162-hoogeboom22a}. 

For use in a predictive setting, the coordinate updates in the diffusion model were turned off and a predictive pooling head was added. 

\subsection{Transfer learning}

We match the backbones of the pre-trained models to freshly initialized models (the pooling heads are not matched, they remain randomly initialized). The backbone is then trained until convergence using early stopping at a learning rate or $5\times10^{-4}$. The backbone is then unfrozen and the entire model is fine-tuned at a lower learning rate $1\times10^{-4}$.

\subsection{Training resources}

Each EGNN model training takes $\sim$6 hours on a single A10 GPU.

\section{Additional split information}

\begin{table}[h]
\centering  
\caption{Overview of UniProt overlap in prevously proposed splits. The numbers denote the number of unique overlapping UniProts, overlapping test structures (out of total test structures), and overlapping train structures (out of total train structures).}
\begin{tabular}{lccc}  
\toprule  
\textbf{Split name} & \textbf{\# UniProts overlap} & \textbf{\# train overlap} & \textbf{\# test overlap} \\  
\midrule  
Post 2019 set (\cite{volkov2022frustration}) & 262 &  5520 / 16561 & 1004 / 1467 \\
CASF 2016 (\cite{volkov2022frustration}) & 67 &  3944 / 16561 & 281 / 282 \\
Zero-Ligand-Bias (\cite{durant2023robustly}) & 170 &  3724 / 17605 & 287 / 360 \\
LeakProof \pdbbind (\cite{li2024leakproofpdbbindreorganized}) & 172 &  1735 / 12923 & 3526 / 4751 \\
\oursplit (Ours) & 0 & 0 / 11022 & 0 / 1857 \\
\bottomrule  
\end{tabular}
\label{table::overlap-table}
\end{table}

\begin{table}[h]  
\centering  
\caption{\casestudy}  
\begin{tabular}{lccc}  
\toprule  
\textbf{UniProt} & \textbf{HGNC} & \textbf{Number of structures} \\  
\midrule  
P00734 & F2           & 170 \\
P56817 & BACE1        & 343 \\
P24941 & CDK2         & 248 \\
O60885 & BRD4         & 199 \\
P00918 & CA2          & 425 \\
P07900 & HSP90AA1     & 172 \\
Q9H2K2 & TNKS2        & 113 \\
P00760 & N/A (Bovine) & 187 \\
\bottomrule  
\end{tabular}  
\end{table}


\section{Metrics}

Below are the explicit equations for the metrics used in the benchmarks

\begin{equation*}
    \textnormal{Pearson Correlation Coefficient} = \frac{\sum_{i} (x_i - \bar{x})(y_i - \bar{y})}{\sqrt{\sum_{i} (x_i - \bar{x})^2} \sqrt{\sum_{j} (y_j - \bar{y})^2}}
\end{equation*}

\begin{equation*}
    R^2 = 1 - \frac{\sum_{i} (x_i - y_i)^2}{\sum_{j} (y_j - \bar{y})^2}
\end{equation*}

\section{Additional plots}

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\textwidth]{plots/combined_rmse.png} 
  \caption{Overall and stratified performance at increasing train data fraction for different model families. In the low data regime, global 3D models outperform local models. Left: The error bars denote the standard deviation across the 3 test folds. Right: The boxplots represent the performance distribution over the eight proteins in the \casestudy set.}
\end{figure}

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\textwidth]{plots/num_train_scatter_rmse.png} 
  \caption{Effect of number of training data points on performance. Each point represents a protein from the 8 case-study proteins. The global models show a clear advantage at low data regimes.}
\end{figure}


\begin{figure}[!htb]
  \centering
  \includegraphics[width=\textwidth]{plots/gnn_combined_rmse.png} 
    \caption{Effect of the EGNN additions proposed in this study on model performance. The overall performance across all eight proteins in the \casestudy set is reported. The error bars denote the standard deviation across the 3 test folds. \textbf{Pre-training}: Quantum mechanical pre-training provides the greatest advantage, followed closely by diffusion pre-training.
  \textbf{Hydrogens}: Including explicit hydrogens is very important at low data levels.
  \textbf{Interacting pose}: No consistent pattern becomes apparent when comparing single-graph versus multi-graph. }
\end{figure}

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\textwidth]{plots/combined_pearson.png} 
  \caption{Overall and stratified performance at increasing train data fraction for different model families. In the low data regime, global 3D models outperform local models. Left: The error bars denote the standard deviation across the 3 test folds. Right: The boxplots represent the performance distribution over the eight proteins in the \casestudy set.}
\end{figure}

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\textwidth]{plots/num_train_scatter_pearson.png} 
  \caption{Effect of number of training data points on performance. Each point represents a protein from the 8 case-study proteins. The global models show a clear advantage at low data regimes.}
\end{figure}


\begin{figure}[!htb]
  \centering
  \includegraphics[width=\textwidth]{plots/gnn_combined_pearson.png} 
    \caption{Effect of the EGNN additions proposed in this study on model performance. The overall performance across all eight proteins in the \casestudy set is reported. The error bars denote the standard deviation across the 3 test folds. \textbf{Pre-training}: Quantum mechanical pre-training provides the greatest advantage, followed closely by diffusion pre-training.
  \textbf{Hydrogens}: Including explicit hydrogens is very important at low data levels.
  \textbf{Interacting pose}: No consistent pattern becomes apparent when comparing single-graph versus multi-graph. }
\end{figure}
